Stability Analysis and Generalization Bounds of Adversarial Training

In adversarial machine learning, deep neural networks can fit the adversarial examples on the training dataset but have poor generalization ability on the test set. This phenomenon is called robust overfitting, and it can be observed when adversarially training neural nets on common datasets, including SVHN, CIFAR-10, CIFAR-100, and ImageNet. In this paper, we study the robust overfitting issue of adversarial training by using tools from uniform stability. One major challenge is that the outer function (as a maximization of the inner function) is nonsmooth, so the standard technique (e.g., hardt et al., 2016) cannot be applied. Our approach is to consider $\eta$-approximate smoothness: we show that the outer function satisfies this modified smoothness assumption with $\eta$ being a constant related to the adversarial perturbation $\epsilon$. Based on this, we derive stability-based generalization bounds for stochastic gradient descent (SGD) on the general class of $\eta$-approximate smooth functions, which covers the adversarial loss. Our results suggest that robust test accuracy decreases in $\epsilon$ when $T$ is large, with a speed between $\Omega(\epsilon\sqrt{T})$ and $\mathcal{O}(\epsilon T)$. This phenomenon is also observed in practice. Additionally, we show that a few popular techniques for adversarial training (e.g., early stopping, cyclic learning rate, and stochastic weight averaging) are stability-promoting in theory.

==> intro.tex <==
\section{Introduction}

The most widely used optimization method in machine learning practice is
\emph{stochastic gradient method} (SGM). Stochastic gradient methods aim to
minimize the empirical risk of a model by repeatedly computing the gradient of
a loss function on a single training example, or a batch of few examples, and
updating the model parameters accordingly. SGM is scalable, robust, and
performs well across many different domains ranging from smooth and strongly
convex problems to complex non-convex objectives.

In a nutshell, our results establish that:
\submit{
\emph{Any model trained with stochastic gradient method
in a reasonable amount of time attains small generalization error.}
}{
\begin{center}
\emph{Any model trained with stochastic gradient method
in a reasonable\\ amount of time attains small generalization error.}
\end{center}
} % end submit

As training time is inevitably limited in practice, our results help to
explain the strong generalization performance of stochastic gradient methods
observed in practice. More concretely, we bound the generalization error of
a model in terms of the number of iterations that stochastic gradient method
took in order to train the model. Our main analysis tool is to employ the
notion of algorithmic stability due to Bousquet and
Elisseeff~\citeyr{BousquetE02}. We demonstrate that the stochastic
gradient method is stable provided that the objective is relatively smooth
and the number of steps taken is sufficiently small.

It is common in practice to perform a linear number of steps in the size of
the sample and to access each data point multiple times. Our results show in
a broad range of settings that, provided the number of iterations is linear
in the number of data points, the generalization error is bounded by a
vanishing function of the sample size. The results hold true even for
complex models with large number of parameters and no explicit
regularization term in the objective. Namely, fast training time by itself
is sufficient to prevent overfitting.

Our bounds are algorithm specific: Since the number of iterations we allow
can be larger than the sample size, an arbitrary algorithm could easily
achieve small training error by memorizing all training data with no
generalization ability whatsoever. In contrast, if the stochastic gradient
method manages to fit the training data in a reasonable number of
iterations, it is guaranteed to generalize.

Conceptually, we show that minimizing training time is not only beneficial
for obvious computational advantages, but also has the important
byproduct of decreasing generalization error. Consequently, it may make
sense for practitioners to focus on minimizing training time, for instance,
by designing model architectures for which stochastic gradient method
converges fastest to a desired error level.


\subsection{Our contributions}

Our focus is on generating \emph{generalization bounds} for models learned with stochastic gradient descent.  Recall that the generalization bound is the expected difference between the error a model incurs on a training set versus the error incurred on a new data point, sampled from the same distribution that generated the training data.  Throughout, we assume we are training models using $n$ sampled data points.

Our results build on a fundamental connection between the generalization error
of an algorithm and its \emph{stability} properties.  Roughly speaking, an
algorithm is \emph{stable} if the training error it achieves varies only
slightly if we change any single training data point. The precise notion of
stability we use is known as \emph{uniform stability} due
to~\cite{BousquetE02}. It states that a randomized algorithm~$A$ is uniformly
stable if for all data sets differing in only one element, the learned models produce nearly the same predictions.   We review this method in Section~\ref{updates:sec}, and provide a new adaptation of this theory to \emph{iterative} algorithms.

In Section~\ref{sec:sgd}, we show that stochastic gradient is uniformly stable, and our techniques mimic its convergence proofs.  For convex loss functions, we prove that the stability measure decreases as a function of the sum of the step sizes.  For strongly convex loss functions, we show that stochastic gradient is stable, even if we train for an arbitrarily long time.   We can combine our bounds on the generalization error of stochastic gradient
method with optimization bounds quantifying the convergence of the empirical
loss achieved by SGM. In Section~\ref{sec:case-studies}, we show that models trained for multiple epochs match classic bounds for stochastic gradient~\cite{NY78,NY83}.  
%
%We also show how regularization allows to train with stochastic gradient descent for an arbitrarily long time without fear of overfitting. Moreover, we show that regularization removes the need for model averaging in order to obtain optimal sample complexity bounds for learning.
%

More surprisingly, our results carry over to the case where the loss-function is non-convex.  In this case we show that the method generalizes provided the steps are sufficiently small and the number of iterations is not too large.  More specifically, we show the number of steps of stochastic gradient can grow as $n^c$ for a small $c>1$.  This provides some explanation as to why neural networks can be trained for  multiple epochs of stochastic gradient and still exhibit excellent generalization.
In Section~\ref{sec:operations}, we furthermore show that various heuristics used in practice, especially in the deep learning community, help to increase the stability of stochastic gradient method. 
%
For example, the popular dropout scheme~\cite{krizhevsky2012imagenet,srivastava2014dropout} 
%decreases the parameter~$L$ proportionally to the dropout probability thus 
improves all of our bounds. Similarly, $\ell_2$-regularization improves the exponent of $n$ in our non-convex result. In
fact, we can drive the exponent arbitrarily close to $1/2$ while preserving the
non-convexity of the problem. 


\subsection{Related work}

There is a venerable line of work on stability and generalization dating back
more than thirty
years~\cite{DevroyeW79,KearnsR99,BousquetE02,MukherjeeNPR06,SSSS10}.  The
landmark work by Bousquet and Elisseeff~\cite{BousquetE02} introduced the
notion of \emph{uniform stability} that we rely on. They showed that several
important classification techniques are uniformly stable. In particular, under certain regularity assumptions, it
was shown that the \emph{optimizer} of a regularized empirical loss
minimization problem is uniformly stable.  Previous work generally applies only to
the exact minimizer of specific optimization problems.  It is not immediately evident on how to compute a generalization bound for an approximate minimizer such as one found by using stochastic gradient.  Subsequent work studied stability bounds for randomized algorithms but focused on random perturbations of the cost function, such as those induced by bootstrapping or bagging~\cite{Elisseeff05}.  This manuscript differs from this foundational work in that it derives stability bounds about the learning \emph{procedure}, analyzing algorithmic properties that induce stability.

Stochastic gradient descent, of course, is closely related to our inquiry.  
Classic results by Nemirovski and Yudin show that the stochastic gradient 
method produces is nearly optimal for empirical risk minimization of convex loss functions~\cite{NY78,  NY83, Nemirovski09,frostig15competing}.  These results have been extended by many machine learning researchers, yielding tighter bounds and probabilistic guarantees ~\cite{Hazan06,HazanKale14, Rakhlin11}.  However, there is an important limitation of all of this prior art.  The derived generalization bounds only hold for single passes over the data.  That is, in order for the bounds to be valid, each training example must be used no more than once in a stochastic gradient update.  In practice, of course, one tends to run multiple \emph{epochs} of the stochastic gradient method.	Our results resolve this issue by combining stability with optimization error.  We use the foundational results to estimate the error on the \emph{empirical risk} and then use stability to derive a deviation from the true risk.  This enables us to study the risk incurred by multiple epochs and provide simple analyses of regularization methods for convex stochastic gradient.  We compare our results to this related work in Section~\ref{sec:case-studies}.  We note that Rosasco and Villa obtain risk bounds for least squares minimization with an incremental gradient method in terms of the number of epochs~\cite{Rosasco14}. These bounds are akin to 
our study in Section~\ref{sec:case-studies}, 
although our results are incomparable due to various different assumptions.

Finally, we note that in the non-convex case, the stochastic gradient method is remarkably successful for training large neural networks~\cite{Bottou98, krizhevsky2012imagenet}.  However, our theoretical understanding of this method is limited.  Several authors have shown that the stochastic gradient method finds a stationary point of nonconvex cost functions~\cite{KushnerBook,ghadimi2013stochastic}.  Beyond asymptotic convergence to stationary points, little is known about finding models with low training or generalization error in the nonconvex case.   There have recently been several important studies investigating optimal training of neural nets.  For example Livni \emph{et al.} show that networks with polynomial activations can be learned in a greedy fashion~\cite{livni2014computational}.  Janzamin \emph{et al.}~\cite{Janzamin15} show that two layer neural networks can be learned using tensor methods. Arora~\emph{et al.}~\cite{Arora15} show that two-layer sparse coding dictionaries can be learned via stochastic gradient. Our work complements these developments: rather than providing new insights into mechanisms that yield low training error, we provide insights into mechanisms that yield low generalization error. If one can achieve low training error quickly on a nonconvex problem with stochastic gradient, our results guarantee that the resulting model generalizes well.

